Switch as a Verifier: Toward Scalable Data Plane Checking via Distributed, On-Device Verification

Data plane verification (DPV) is important for finding network errors. Current DPV tools employ a centralized architecture, where a server collects the data planes of all devices and verifies them. Despite substantial efforts on accelerating DPV, this centralized architecture is inherently unscalable. In this paper, to tackle the scalability challenge of DPV, we circumvent the scalability bottleneck of centralized design and design Coral, a distributed, on-device DPV framework. The key insight of Coral is that DPV can be transformed into a counting problem on a directed acyclic graph, which can be naturally decomposed into lightweight tasks executed at network devices, enabling scalability. Coral consists of (1) a declarative requirement specification language, (2) a planner that employs a novel data structure DVNet to systematically decompose global verification into on-device counting tasks, and (3) a distributed verification (DV) protocol that specifies how on-device verifiers communicate task results efficiently to collaboratively verify the requirements. We implement a prototype of Coral. Extensive experiments with real-world datasets (WAN/LAN/DC) show that Coral consistently achieves scalable DPV under various networks and DPV scenarios, i.e., up to 1250 times speed up in the scenario of burst update, and up to 202 times speed up on 80% quantile of incremental verification, than state-of-the-art DPV tools, with little overhead on commodity network devices.

==> Wen.tex <==
\section{Performance Evaluation Plan}~\label{sec:eval}

\begin{table}[!htbp]
    \centering
\footnotesize
    \begin{tabular}{|c|c|c|c|c|c}
	        \hline
        \textbf{Network} & \textbf{\#Devices} & \textbf{\#Links} & \textbf{\#Rules} \\
        \hline
	\lnet{} & 6,016 & 43,008 & $3.2 \times 10^7$ \\
        \hline
	    Fattree ($k=48$) & 2,880 & 55,296 & $3.31 \times 10^6$ \\
        \hline
        Internet2 & 9 & 28 & $1.26 \times 10^5$ \\
        \hline
        Stanford & 16 & 74 & $3.84 \times 10^3$ \\
        \hline
         xxxx &  &  &  \\
        \hline
         yyyy &  &  &  \\
        \hline
    \end{tabular}
    \caption{The datasets used in the evaluation.}
    \label{tab:datasets}
\end{table}


\begin{table}[t]
    \centering
\footnotesize
    \begin{tabular}{|c|c|c|c|}
    \hline
        \textbf{Network} & \textbf{APKeep} & \textbf{\system} & \textbf{Ratio} \\
        \hline
	    \lnet{} & 111,558.276 & 40.442 & $2,758\times$ \\
        \hline
        Fattree & 3,293.302 & 4.042 & $815\times$ \\
        \hline
        Internet2 & 3.728 & 0.283 & $13\times$ \\
        \hline
        Stanford & 0.403 & 0.082 & $5\times$ \\
        \hline
        xxxx &  &  &  \\
        \hline
        yyyy &  &  &  \\
        \hline
    \end{tabular}
    \caption{The verification time of burst update (seconds).}
    \label{tab:green-start}
\end{table}


\begin{table}[t]
    \centering
\footnotesize
    \begin{tabular}{|c|c|c|c|c|c|c}
    \hline
        \textbf{Network} & \textbf{DDPV} & \textbf{APKeep}\\
	    \ & mean median& mean median\\
        \hline
	    \lnet{} &  & \\
        \hline
        Fattree &  &\\
        \hline
        Internet2 & & \\
        \hline
        Stanford & &\\
        \hline
        xxxx &  &\\
        \hline
        yyyy & & \\
        \hline
    \end{tabular}
    \caption{Average and median run time of DDPV and APkeep, for a single rule update (seconds).}
    \label{tab:green-start}
\end{table}


\begin{table}[t]
    \centering
\footnotesize
    \begin{tabular}{|c|c|c|c|c|c|c}
    \hline
        \textbf{Network} & \textbf{mean} & \textbf{median}\\
        \hline
	    \lnet{} &  & \\
        \hline
        Fattree &  &\\
        \hline
        Internet2 & & \\
        \hline
        Stanford & &\\
        \hline
        xxxx &  &\\
        \hline
        yyyy & & \\
        \hline
    \end{tabular}
    \caption{Average and median run time of node of DDPV for a single rule update.}
    \label{tab:green-start}
\end{table}




\begin{figure*}[t]
    \centering
	\begin{subfigure}[t]{0.25\linewidth}
	    \centering\includegraphics[width=1\linewidth]{figures/eval/inc_fb.png}
		\caption{\label{fig:eval-inc-fb} \lnet.}
	\end{subfigure}
\hfill
	\begin{subfigure}[t]{0.25\linewidth}
	    \centering\includegraphics[width=1\linewidth]{figures/eval/inc_ft.png}
		\caption{\label{fig:eval-inc-ft} Fattree.}
	\end{subfigure}
\hfill
	\begin{subfigure}[t]{0.25\linewidth}
	    \centering\includegraphics[width=1\linewidth]{figures/eval/inc_i2.png}
		\caption{\label{fig:eval-inc-i2} Internet2.}
	\end{subfigure}
    \caption{The incremental verification time (microseconds).}
\end{figure*}

\begin{figure*}[t]
	\begin{subfigure}[t]{0.25\linewidth}
	    \centering\includegraphics[width=1\linewidth]{figures/eval/inc_st.png}
		\caption{\label{fig:eval-inc-st} Stanford.}
	\end{subfigure}
\hfill
	\begin{subfigure}[t]{0.25\linewidth}
	    \centering\includegraphics[width=1\linewidth]{new_tem/incremental_DDPV_APkeep.png}
		\caption{\label{fig:incremental DDPV APkeep} xxxx.}
	\end{subfigure}
\hfill
	\begin{subfigure}[t]{0.25\linewidth}
	    \centering\includegraphics[width=1\linewidth]{new_tem/incremental_DDPV_APkeep.png}
		\caption{\label{fig:incremental DDPV APkeep} yyyy.}
	\end{subfigure}
    \caption{The incremental verification time (microseconds).}
\end{figure*}

\begin{figure*}[b]
    \centering
	\begin{subfigure}[t]{0.25\linewidth}
	    \centering\includegraphics[width=0.5\linewidth]{new_tem/Exchanged_message_size.png}
		\caption{\label{fig:eval-inc-fb} Exchanged message size.}
	\end{subfigure}
\hfill
	\begin{subfigure}[t]{0.25\linewidth}
	    \centering\includegraphics[width=0.5\linewidth]{new_tem/Number_of_exchnaged_message.png}
		\caption{\label{fig:eval-inc-ft} Number of exchnaged message.}
	\end{subfigure}
    \caption{Exchanged message for an incremental verification.}
\end{figure*}

\begin{figure}[!htbp]
\centering
\includegraphics[width=0.4\textwidth]{new_tem/time_of_key_step.png}
\caption{\label{fig:dataplane}Time of key step for an incremental verification (microseconds).}
\end{figure}

\begin{figure}[!htbp]
\centering
\includegraphics[width=0.4\textwidth]{new_tem/CIB.png}
\caption{\label{fig:dataplane}Number of CIB.}
\end{figure}


\begin{figure}[t]
   \centering
	\begin{subfigure}[t]{0.48\linewidth}
	    \centering\includegraphics[width=1\linewidth]{figures/eval/memory.png}
		\caption{\label{fig:eval-micro-mem} Memory consumption.}
	\end{subfigure}
%\hfill
%	\begin{subfigure}[t]{0.24\linewidth}
%	    \centering\includegraphics[width=1\linewidth]{figures/eval/cib.png}
%		\caption{\label{fig:eval-micro-cib} Number of entries in CIB}
%	\end{subfigure}
\hfill
	\begin{subfigure}[t]{0.48\linewidth}
	    \centering\includegraphics[width=1\linewidth]{figures/eval/msg.png}
		\caption{\label{fig:eval-micro-size} Message size.}
	\end{subfigure}
    \caption{The overhead of \system{}.}
\end{figure}


==> abstract.tex <==
\begin{abstract}
	Data plane verification (DPV) is an important tool for ensuring the
	correctness of networks. Existing DPV tools take a centralized design,
	where a controller collects all the FIB and performs the verification.
	Despite substantial efforts on how to accelerate DPV, this design is
	inherently unscalable. In this paper, we take a radically different approach to
	design a  distributed data plane verification (\system{}) framework to
	achieve scalable, real-time verification of network data planes.  Our key
	observation is that the job of verifying a global property of a network
	can be transformed into a counting problem on a directed acyclic graph,
	which can be decomposed into smaller tasks distributed to and executed
	at devices, enabling low-latency and scalability.  In \system{}, we
	provide a declarative language for specifying global properties to
	verify. We develop a decomposition engine that decomposes a global
	property into smaller tasks to be executed at devices and specifies
	their execution dependencies. We design an efficient distributed
	verification protocol that executes the decomposed tasks subject to
	their dependencies to compute the verification result. We implement a
	prototype of \system{} and conduct extensive experiments on real data
	plane datasets and topologies. Our results show XXX.
\end{abstract}

\iffalse
 One exception is RCDC, in which each switch
	performs local verification, but it can only verify a very specific
	requirement.
\fi










==> architecture.tex <==
\begin{figure}[t]
%\setlength{\abovecaptionskip}{0.1cm}
%\setlength{\belowcaptionskip}{-0.cm}
\centering
\includegraphics[width=0.9\columnwidth]{figures/ddpv-architecture-v1.pdf}
\caption{The architecture and basic workflow of \system{}.}
\label{fig:arch}
%\reducespace
%\vspace{-1em}
\end{figure}

\subsection{Architecture}\label{sec:arch}
Figure~\ref{fig:arch} gives the architecture of \system{}.
\system{} is composed of a centralized verification planner and on-device
verifiers residing on network devices. 

\para{Verification planner.} 
This component is logically centralized. It takes in a verification
requirement specified using the \system{} specification
language~(Section~\ref{sec:lang}), and the topology and device-IP prefix mapping
information of the topology, and decides the on-device verification tasks for
each network device to perform distributed verification. To this end, the
planner first leverages the automata theory~\cite{lewis1998elements} to take the product of 
the regular expression $path$ in the requirement and the network topology, and
gets a DAG termed \dvnet{} as the result. Similar to the logical topology in
Merlin~\cite{merlin} and the product graph in Contra~\cite{contra}, a \dvnet{} 
compactly represents
all paths in the topology that are allowed by the requirement. It is decided
only by the verification requirement and the topology, and is independent
of the actual data plane of the network. \qiao{added this sentence to clarify
\dvnet{} has nothing to do with FIB.}

With \dvnet{}, the planner is able to transform the problem of data plane
verification into a counting problem on \dvnet{}: \textit{given a packet
$p$, is there a satisfactory number of copies of $p$ delivered to the
destination node of the DVNet in each universe? \qiao{XX}} 

Directly counting on \dvnet{}, however, requires collecting the
data planes of all devices, which is still centralized and not scalable.
\qiao{change first sentence if we change the story to on-device verification, or
we call it in-network verification?} As such, the
planner further decomposes the counting problem into smaller on-device counting tasks, one for each node in \dvnet{}. 
Given a node $u$ in \dvnet{}, 
its on-device counting task takes in the counting task results of all $u$'s downstream neighbors, as well as the data plane of $u$'s residing device, counts the number of packet copies that can reach from $u$ to the destination node in \dvnet{}. These tasks are sent to the corresponding devices in the
network topology, together with device-to-device communication instructions,
and executed in a distributed manner to compute the final verification result. 

\begin{figure*}[h]
    \centering
	\begin{subfigure}[t]{0.36\linewidth}
	    \centering\includegraphics[width=0.95\linewidth]{figures/workflow-topo-v5.pdf}
		\caption{\label{fig:workflow-topo} An example network topology
		and requirement.}
	\end{subfigure}
\hfill
	\begin{subfigure}[t]{0.23\linewidth}
	    \centering\includegraphics[width=0.95\linewidth]{figures/workflow-fib-v3.pdf}
		\caption{\label{fig:workflow-fib} The data plane.}
	\end{subfigure}
\hfill
	\begin{subfigure}[t]{0.38\linewidth}
	    \centering\includegraphics[width=0.95\linewidth]{figures/workflow-dvnet-v4.pdf}
		\caption{\label{fig:workflow-dvnet} The \dvnet{} and the counting process.}
	\end{subfigure}
    \caption{An illustration example to demonstrate the workflow of \system{}.}
    \label{fig:workflow-example}
\end{figure*}



\para{On-device verifier equipped with the DV protocol.}
Given a network device, its on-device verifier receives the counting tasks
from the verification planner, executes them, and sends the counting results to
corresponding neighboring devices based on the predefined communication
instructions from the planner. To this end, we design
a DV protocol that specifies how on-device verifiers
compute and incrementally update their on-device tasks, as well as how they
communicate the results to neighbors efficiently and correctly. 

In a nutshell, to execute an on-device counting task, the on-device verifier
first reads the device's data plane and constructs a table of local equivalence
classes (LECs).  Informally, an LEC at device $X$ is a set of packets whose
actions are identical at $X$. \qiao{needs a formal definition or not?} Computing and maintaining the LEC table can be
realized using existing DPV tools~(\eg, DeltaNet~\cite{deltanet-nsdi17},
VeriFlow~\cite{veriflow}, AP~\cite{ap-icnp13} and APKeep~\cite{apkeep-nsdi20}) 
by considering $X$ the only device in the network. 

Next, the on-device verifier uses the LEC table and the results of other tasks
sent from neighboring devices as input, and counts, across the packet space,
the number of packet copies that can reach the destination node in \dvnet{} from the current node. The results are stored in a counting information
base (CIB) and sent to the on-device verifiers at neighboring devices
incrementally, based on the device-to-device communication instructions
specified by the planner and the DV protocol. 


%~\qiao{rewrite this part after finishing section 4.}















==> backup.tex <==
\begin{algorithm}[h]
	$CIB2Change(u) \leftarrow \emptyset$\;
	\If{$CIBIn(v).WID = \emptyset$}{
		$CIB2Change(u) \leftarrow CIB(u)$\;
	}
	\Else{
		\ForEach{entry $r$ in $CIB(u)$}{
			\If{$\exists wid \in CIBIn(v).WID: wid \in r.history$}{
				$CIB2Change(u) \leftarrow CIB2Change(u) \cup \{r\}$\;
			}
		}
	}
	$CIBChange(u) \leftarrow $ {\sc getCIBChange$(CIB2Change(u), CIBIn(v).Table)$}\;
	$CIB(u) \leftarrow (CIB(u) - CIB2Change(u)) \cup CIBChange(u)$\;
	$WID \leftarrow CIB2Change(u).ID$\;
	$CIBOut(u) \leftarrow (CIBChange(u), WID)$\;
	\caption{{\sc CIBUpdate}$(u, CIBIn(v))$}
	\label{alg:cib-update}
\end{algorithm}

\begin{algorithm}[t]
	$CIBChange(u) \leftarrow \emptyset$\;
	\ForEach{entry $r$ in $CIB2Change(u)$}{
		\ForEach{entry $r'$ in $CIBIn(v).Table;$}{
			$r^{new}.pred \leftarrow r.pred \cap r'.pred$\;
			\If{$r^{new}.pred \neq \emptyset$}{
				$r^{new}.action \leftarrow r.action$\;
					$r^{new}.cnt \leftarrow r.cnt - v.cnt + r'.cnt$\;
					$r^{new}.history \leftarrow r.history - \{(v, v.cnt)\} \cup \{(v, r'.cnt)\}$\;
				}
				$r.pred \leftarrow r.pred - r^{new}.pred$\;
				$CIBChange(u) \leftarrow CIBChange(u) \cup \{r^{new}\}$\;
			}
					
		}
	\textbf{Return} $CIBChange(u)$\;	
	\caption{{\sc getCIBChange$(CIB2Change(u), CIBIn(v).Table)$} \qiao{only
ALL is considered, ANY is not added yet.}}
	\label{alg:entry-update}
\end{algorithm}


\begin{algorithm}[t]
	$CIB2Change(u) \leftarrow \emptyset$\;
        \ForEach{entry $r'$ in $CIB(u)$}{
		\If{$\exists r'.id \in FIBHistory(f):$}{
			$CIB2Change(u) \leftarrow CIB2Change(u) \cup \{r\}$\;
		}
	}
	\textbf{Return} $CIB2Change(u)$\;
	\caption{{\sc getCIB2ChangeOfFIB}$f$}
	\label{alg:fib-update}
\end{algorithm}


\begin{algorithm}[t]
	$CIBChange(u) \leftarrow \emptyset$\;
	$tmp(r) \leftarrow \emptyset$\;
    \ForEach{entry $r$ in $FIBChange(u)$}{
        \If{$r.pred \neq \emptyset$}{
        $CIB2Change(u) \leftarrow CIB2Change(u) \cup $ {\sc getCIB2ChangeOfFIB$(r)$}\;
		$tmpCib(r) \leftarrow cibOfr$\;
		\ForEach{entry $act$ in $r.action$}{
		    \ForEach{entry $cib$ in $tmpCib(r)$}{
		        \ForEach{entry $r'$ in $CIBIn(act).Table;$}{
			        $r^{new}.pred \leftarrow cib.pred \cap r'.pred$\;
			        \If{$r^{new}.pred \neq \emptyset$}{
				        $r^{new}.action \leftarrow cib.action$\;
					    $r^{new}.cnt \leftarrow cib.cnt + r'.cnt$\;
					    $r^{new}.history \leftarrow cib.history  \cup \{(act, r'.cnt)\}$\;
					    $CIBChange(u) \leftarrow CIBChange(u) \cup \{r^{new}\}$\;
					    $tmp(r) \leftarrow tmp(r)  \cup \{r^{new}\}$\;
				    }
			    }
	        }
	        $tmpCib(r) \leftarrow tmp(r)$\;
	        $tmp(r) \leftarrow \emptyset$\;
	    }
	    }
	}
	$CIB(u) \leftarrow (CIB(u) - CIB2Change(u)) \cup CIBChange(u)$\;
	$WID \leftarrow CIB2Change(u).ID$\;
	$CIBOut(u) \leftarrow (CIBChange(u), WID)$\;
	\caption{{\sc FIBUpdate}$(FIBChange(u)$,CIB(u))}
	\label{alg:fib-update}
\end{algorithm}

\begin{algorithm}[t]
	$delCIB \leftarrow \emptyset$\;
	$lecChange \leftarrow \emptyset$\;
	$CIBChange \leftarrow \emptyset$\;
    \ForEach{entry $c$ in $Change(u)$}{
        $intersectPre \leftarrow c.pred \cap requirement.packetSpace$\;
        \If{$intersectPre \neq \emptyset$}{
		    $tmpCib \leftarrow CIB$\;
		    \If{$ c.newPort \in needNextPionter(u)$ or $ c.oldPort \in needNextPionter(u)$}{
		        \ForEach{entry $r$ in $tmpCib$}{
		            \If{$ c.newPort \in r.action$ or $ c.oldPort \in r.action$}{
		                $delCIB \leftarrow delCIB \cup r$\;
		            }
		        }
		        \If{$c.newPort$ noin $needNextPionter(u)$}{
		            \ForEach{entry $r$ in $tmpCib$}{
		                \If{$r.action \leftarrow \emptyset$}{
		                    $CIB \leftarrow CIB - r $\;
		                    $r.predicate \leftarrow r.predicate \cup c.predicate$\;
		                    $CIB \leftarrow CIB + r $\;
		                    $WID \leftarrow r.id $\;
		                    $CIBChange \leftarrow r$\;
		                }
		            }
		        }
		        \If{$c.oldPort$ noin $needNextPionter(u)$}{
		            \ForEach{entry $r$ in $tmpCib$}{
		                \If{$r.action \leftarrow \emptyset$}{
		                    $CIB \leftarrow CIB - r $\;
		                    $r.predicate \leftarrow r.predicate - c.predicate$\;
		                    $CIB \leftarrow CIB + r $\;
		                    $WID \leftarrow r.id $\;
		                    $CIBChange \leftarrow r$\;
		                }
		            }
		        }
		        \ForEach{entry $f$ in $LEC(u)$}{
		            $interPre \leftarrow f.pred \cap requirement.packetSpace$\;
		            \If{$interPre \neq \emptyset$}{
		                \If{$c.newPort \in f.needNextPointer$ or $c.oldPort \in f.needNextPointer$}{
		                    $lecChange \leftarrow lecChange \cup f$\;
		                }
		            }
		        }
	        }
	    } 
	}
	$CIB \leftarrow CIB - delCIB $\;
    $CIBChange \leftarrow CIBChange \cup FIBUpdate(lecChange(u),CIB(u))$\;
    $CIB \leftarrow CIB \cup CIBChange$\;
    
	$WID \leftarrow WID \cup delCIB(u).ID$\;
	$CIBOut(u) \leftarrow (CIBChange(u), WID)$\;
	\caption{{\sc LECUpdate}$(Change(u)$,CIB(u))}
	\label{alg:lec-update}
\end{algorithm}




==> discussion.tex <==
\section{Discussion}

\para{Q: [Packet Transformation]} 
Can \system{} verify a data plane with packet transformations?

\para{A:} Yes, \system{} can verify a data plane with packet transformations. To
this end, \system{} keeps using the BDD-based approach (\eg,
\cite{scalable-ap-ton17}) to encode
packet transformations, and extends the CIB and the DV UPDATE message to
record and share the counting results of packet transformation actions. 

\para{Q: [Huge Number of Paths]}
What if given a requirement, the number of paths satisfying the $path\_set$ is
large, \eg, exponential to the network size? Wouldn't the \dvnet{} become too large to be
useful?

%Won't \dvnet{} have an exponential size in the worst case? 

\para{A:} First, \dvnet{} is very efficient in verifying typical data plane requirements. Specifically, our literature survey
and private conversations with operators suggest that operators usually want the
data plane to provide paths with limited hop count, if not the shortest one. The
number of such paths is small.  In addition, we also perform DFA
minimization to further reduce the size of \dvnet{}. Second, for requirements
with a huge number of valid paths, we can verify them via divide-and-conquer:
divide the network into partitions abstracted as one-big-switches, construct
\dvnet{} on this abstract network, and perform intra- and inter-partition
distributed verifications.



\para{Q: [\system{} Deployment Flexibility]} 
Does \system{} have to be distributively deployed at network devices? 
%verify requirements related to packet transformation?

\para{A:} No, \system{} is much more flexible. One example is the
divide-and-conquer scenario in the last answer. We can deploy one
verifier for each partition. The verifier performs intra-partition verification,
and exchange results with verifiers of other partitions for inter-partition
verification. In the extreme case, \system{} can even be deployed in a cluster of servers as a
centralized verification tool.

\para{Q: [\system{} Limitations]}
What are the limitations of \system{}? In other words, what is difficult for
\system{} to achieve?

\para{A:} First, \system{} currently only supports ``single-path" requirements,
\ie, requirements specifying each trace should satisfy certain patterns. It
cannot verify ``multi-path" requirements, \eg, node-disjoint / link-disjoint
paths. Verifying these requirements may require the help of requirement-related
algorithms, \eg, the Suurballe's algorithm~\cite{suurballe1974disjoint}. Second,
the performance of \system{} highly depends on the representation of predicates.
Compared with BDD, novel data structures (\eg, ddNF~\cite{bjorner2016ddnf} and
\#PEC~\cite{horn2019precise}) may help further improve \system{}'s efficiency.
Third, \system{} does not support verifying stateful (\eg, middlebox) or
programmable (\eg, P4\cite{bosshart2014p4}) data planes. We leave the
investigation of these limitations as future work.









==> facebook.tex <==
\section{Deploying \system{} on Facebook Global Network}


\subsection{Single data center}
\para{Requirements and specifications}.
(1) (Shortest path ToR-to-ToR Reachability): 
For each ToR switch, its associated IP can reach the associated IPs of all
other ToR switches along a shortest path; 
\begin{lstlisting}
reqList=[]
for S, D in TOR:
  if isSamePod(S, D):
    req=(srcIP=S.IP and dstIP=D.IP, 
         [S], S.D, "exists >= 1")
  else:
    req=(srcIP=S.IP and dstIP=D.IP, 
           [S], S...D, "exists >= 1")
  reqList.add(req)
\end{lstlisting}

(2) (ECMP Shortest path ToR-to-ToR Reachability):
For each ToR switch, its associated IP can reach the associated IPs of all
other ToR switches along all shortest paths (\ie, ECMP); 
\begin{lstlisting}
reqList=[]
for S, D in TOR:
  if isSamePod(S, D):
    req=(srcIP=S.IP and dstIP=D.IP, 
         [S], S.D, "equal")
  else:
    req=(srcIP=S.IP and dstIP=D.IP, 
           [S], S...D, "equal")
  reqList.add(req)
\end{lstlisting}

(3) (Shortest path ToR-to-PR Reachability):
For each ToR switch, its associated IP can reach all external IPs through at
least one PR (peering router) along a shortest path;
\begin{lstlisting}
reqList=[]
for S in TOR:
  req=[]
  for D in PR:
    req=req or (srcIP=S.IP and dstIP=extIP, 
        [S], S...D, "exists >= 1")
  reqList.add(req)
\end{lstlisting}

(4) (Shortest path PR-to-ToR Reachability):
For each PR, its associated external IP can reach all associated IPs of all
ToR switches along a shortest path. 
\begin{lstlisting}
reqList=[]
for S in PR:
  for D in TOR:
    req=(srcIP=extIP and dstIP=D.IP, 
           [S], S...D, "exists >= 1")
    reqList.add(req) 
\end{lstlisting}

Note that similar to (1), (3) and (4) can also be changed to the ``equal"
context. 


(5) 
(ECMP Shortest path ToR-to-ToR Reachability against FSW-RSW failure):
\begin{lstlisting}
reqList=[]
for S, D in TOR:
  if not isSamePod(S, D):
    req=(srcIP=S.IP and dstIP=D.IP, 
         [S], S.D, "equal")

  reqList.add(req)
\end{lstlisting}









==> fig10_11.tex <==
\section{Initialization and trace data}

\textbf{initialization}

number of routers: 376

(1) total time (s)

mellanox max time: 0.897269599

barefoot max time: 1.525707217

edgecore max time: 0.680962295

(2) memory (MB)

mellanox max memory: 18.001975059509277

barefoot max memory: 19.625365257263184

edgecore max memory: 18.00135898590088

(3) cpu load

mellanox max cpu load: 0.48457093984055927

barefoot max cpu load: 0.12671119362459743

edgecore max cpu load: 0.25348693955146806

\textbf{trace}

number of messages: 835187

(1) time to process each message (ms)

mellanox max time: 3193.908001

barefoor max time: 1421.61719

edgecore max time: 520.18053

(2) memory (MB)

mellanox max memory: 449.55835723876953

barefoot max memory: 454.8390426635742

edgecore max memory: 448.7547836303711

(3) total tima (s)

mellanox max total time: 9.613874732

barefoot max total time: 2.314566485

edgecore max total time: 2.642152017

(4) cpu load

mellanox max cpu load: 0.4929647527390432

barefoot max cpu load: 0.12375129355995786

edgecore max cpu load: 0.2476335778181748

\begin{figure}
\centering
	\begin{subfigure}{0.48\linewidth}
	    \centering\includegraphics[width=1\linewidth]{figures/eval/trace_message_fb_1000.pdf}
		\caption{\label{fig:trace-message-fb-1000} LoNet.}
	\end{subfigure}
\hfill
	\begin{subfigure}{0.48\linewidth}
	    \centering\includegraphics[width=1\linewidth]{figures/eval/trace_message_ft_1000.pdf}
		\caption{\label{fig:trace-total-time-ft-1000} Fattree.}
	\end{subfigure}
	\caption{1000 messages processing time.}
    \label{fig:trace-message-1000}
\end{figure}


\begin{figure}
\centering
	\begin{subfigure}{0.48\linewidth}
	    \centering\includegraphics[width=1\linewidth]{figures/eval/dc_time.pdf}
		\caption{\label{fig:dc-time} Total time.}
	\end{subfigure}
\hfill
	\begin{subfigure}{0.48\linewidth}
	    \centering\includegraphics[width=1\linewidth]{figures/eval/dc_memory.pdf}
		\caption{\label{fig:dc-memory} Memory.}
	\end{subfigure}
\hfill
	\begin{subfigure}{0.48\linewidth}
	    \centering\includegraphics[width=1\linewidth]{figures/eval/dc_load.pdf}
		\caption{\label{fig:dc-load} CPU load.}
	\end{subfigure}
	\caption{Initialization overhead in data center network.}
    \label{fig:dc-initialization}
\end{figure}




==> figure-combination.tex <==
\begin{table*}[]
    \begin{minipage}[t]{0.7\linewidth}
        \input{incremental-evaluation}
    \end{minipage}
\end{table*}

\begin{figure*}[t]
    \centering
    % \hspace{1.7cm}
    \begin{minipage}[t]{0.49\linewidth}
        \centering
        \begin{subfigure}{0.48\linewidth}
    	    \centering\includegraphics[width=1\linewidth]{figures/eval/init_total_time.pdf}
    		\caption{\label{fig:init-total-time} Total time.}
    	\end{subfigure}
    	\begin{subfigure}{0.48\linewidth}
    	    \centering\includegraphics[width=1\linewidth]{figures/eval/init_memory.pdf}
    		\caption{\label{fig:init-memory} Maximal memory.}
    	\end{subfigure}
    	\begin{subfigure}{0.48\linewidth}
    	    \centering\includegraphics[width=1\linewidth]{figures/eval/init_cpu_load.pdf}
    		\caption{\label{fig:init-cpu-load} CPU load.}
    	\end{subfigure}
    % 	\hspace{1.7cm}
    	\caption{Overhead of reading the device dataplane and computing the
    	initial LEC and CIB.}
    	\label{fig:eval-init}
    \end{minipage}
    \begin{minipage}[t]{0.49\linewidth}
        \centering
    	\begin{subfigure}{0.48\linewidth}
    	    \centering\includegraphics[width=1\linewidth]{figures/eval/trace_message.pdf}
    		\caption{\label{fig:trace-message} Time for each message.}
    	\end{subfigure}
    \hfill
    	\begin{subfigure}{0.48\linewidth}
    	    \centering\includegraphics[width=1\linewidth]{figures/eval/trace_total_time.pdf}
    		\caption{\label{fig:trace-total-time} Total time.}
    	\end{subfigure}
    \hfill
    	\begin{subfigure}{0.48\linewidth}
    	    \centering\includegraphics[width=1\linewidth]{figures/eval/trace_memory.pdf}
    		\caption{\label{fig:trace-memory} Memory.}
    	\end{subfigure}
    \hfill
        \begin{subfigure}{0.48\linewidth}
            \centering\includegraphics[width=1\linewidth]{figures/eval/trace_cpu_load.pdf}
            \caption{\label{fig:trace-cpu-load} CPU load.}
        \end{subfigure}
    	\caption{Overhead of computing incremental.}
    	\label{fig:trace}
    \end{minipage}
\end{figure*}

==> figure-combination2.tex <==
\begin{figure*}[h!tbp]
% \setlength{\abovecaptionskip}{0cm}
% \setlength{\belowcaptionskip}{-0.cm}
%     \centering
    % \hspace{1.7cm}
    % \begin{minipage}[]{0.65\linewidth}
        % \input{green-evaluation}
        % \input{incremental-evaluation}
    % \end{minipage}
    % \begin{minipage}[]{0.32\linewidth}
    %     \centering
    %     \begin{subfigure}{\linewidth}
    % 	   \setlength{\abovecaptionskip}{0cm}
    %         \setlength{\belowcaptionskip}{-0.cm}
    %         \centering\includegraphics[width=.7\linewidth]{figures/eval/init_total_time.pdf}
	   %     \caption{\label{fig:init-total-time} \footnotesize Total time.}
    % 	\end{subfigure}
    % 	\begin{subfigure}{\linewidth}
    % 	   \setlength{\abovecaptionskip}{0cm}
    %         \setlength{\belowcaptionskip}{-0.cm} \centering\includegraphics[width=.7\linewidth]{figures/eval/init_memory.pdf}
    %     	\caption{\label{fig:init-memory}\footnotesize Maximal memory.}
    % 	\end{subfigure}
    % 	\begin{subfigure}{\linewidth}
    %         \setlength{\abovecaptionskip}{0cm}
    %         \setlength{\belowcaptionskip}{-0.cm}
    %         \centering\includegraphics[width=.7\linewidth]{figures/eval/init_cpu_load.pdf}
    % 	    \caption{\label{fig:init-cpu-load} \footnotesize CPU load.}
    % 	\end{subfigure}
    % % 	\hspace{1.7cm}
    % 	\caption{Initialization overhead.}
    % 	\label{fig:eval-init}
    % \end{minipage}
\end{figure*}



==> green-evaluation.tex <==
% \begin{table*}[]
\centering
% \footnotesize
\tiny
\resizebox{1\linewidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
        \textbf{Network} & \textbf{AP} & \textbf{APKeep} &
        \textbf{Delta-net} &
        \textbf{VeriFlow} &
        \textbf{\system} \\
        \hline
        
         Internet2 & 2.07 &
	    2.88 &104.71&
	    93.52 & \textbf{exp: 0.99 (2.09$\times$)}  \textbf{simu: 0.95 (2.18$\times$)}  \\
	    
    %     \multirow{2}{*}{Internet2} & \multirow{2}{*}{2.07} &
	   % \multirow{2}{*}{2.88} & \multirow{2}{*}{104.71} &
	   % \multirow{2}{*}{93.52}  & \textbf{exp: 0.99 (2.09$\times$)}  \\
    %      & & & & & \textbf{simu: 0.95 (2.18$\times$)}  \\
        \hline
        Stanford  & 0.49 & 0.29 & 13.28 & 0.28 & \textbf{0.06 (4.67$\times$)}\\
        \hline
        Airtel1-1  & 0.35 & 1.00 &13.57 & 4.97 & \textbf{0.70 (0.50$\times$)}\\
        \hline
        Airtel2-1  & 0.49  & 1.95 &19.08 & 4.59 & \textbf{1.10 (0.45$\times$)} \\
        \hline
        Airtel1-2  & 0.82 & 2.56 & 50.96 & 391.38 & \textbf{0.72 (1.14$\times$)}\\
        \hline
        Airtel2-2  & 5.93  & 18.23 &237.16 & 549.55 & \textbf{1.60 (3.71$\times$)} \\
        \hline
        B4-2013  & 0.58 & 1.84 & 31.86 & 130.08 & \textbf{0.49 (1.18$\times$)}\\
        \hline
        B4-2018  & 1.19 & 2.94 & 55.71 & 539.73 & \textbf{0.69 (1.72$\times$)}\\
        \hline
        BT North America  & 2.05 & 7.25 & 123.17 & 270.14 & \textbf{0.46 (4.46$\times$)}\\
        \hline
        NTT  & 1.65 & 6.53 & 89.05 & 179.57 & \textbf{0.65 (2.54$\times$)}\\
        \hline
        OTEGlobe  & 7.62 & 41.18 & 442.48 & 3411.59 & \textbf{1.20 (6.35$\times$)}\\
        \hline
        Fattree ($k=48$) & 40608.79 % (38.112)
        & 3293.30  & Time Out & Time Out & \textbf{4.05 (813.16$\times$)}\\
        \hline
	    \lnet{} & 50573.80 % (434.671)
	    & 111,558.28 & Time Out & Time Out & \textbf{ 40.45(1250.28$\times$)}\\
        \hline
    \end{tabular}
    }
    \caption{Verification time of burst update (seconds).}
    \label{fig:green-start2}

% \vspace{-3em}
% \end{table*}

% \begin{figure*}
%     \includegraphics[width=0.5\textwidth,height=0.2\textwidth]{figures/9-1.jpg}
% \caption{Verification time of burst update (seconds).}
% \label{fig:Green-Start}
% \end{figure*}

==> incremental-evaluation.tex <==

% \begin{table*}[]
    \centering
% \footnotesize
\huge
\resizebox{\linewidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
	    \hline
	    \multirow{2}{*}{\textbf{Network}} & 
	    \multicolumn{5}{c|}{Percentage < 10 ms} &
	    \multicolumn{5}{c|}{80\% quantile (milliseconds)}  \\
	    \cline{2-11}
         &  \textbf{AP} & \textbf{APKeep} & \textbf{Delta-Net} & \textbf{VeriFlow} & \textbf{DDPV}
         &  \textbf{AP} & \textbf{APKeep} & \textbf{Delta-Net} & \textbf{VeriFlow} & \textbf{DDPV} \\
        \hline
        \multirow{2}{*}{Internet2} & \multirow{2}{*}{0\%} &
	    \multirow{2}{*}{29.29\%} & \multirow{2}{*}{27.97\%} &
	    \multirow{2}{*}{17.71\%} & \textbf{exp: 81.55\%} & \multirow{2}{*}{2782.10} & \multirow{2}{*}{26.55} & \multirow{2}{*}{36.55}  & \multirow{2}{*}{60.92} & \textbf{ 5.42 (4.90$\times$)} \\
        & & & & & \textbf{simu: 83.63\%} & & & & &  \textbf{8.83 (3.01$\times$)} \\
        \hline
        Stanford & 1.23\% & 99.93\% & 98.73\% & 100\% & \textbf{99.76\%} & 10522.66 & 0.27 & 1.43 & 0.39 & \textbf{0.06 (4.5$\times$)} \\
        \hline
        Airtel1-1 & 0\% & 15.19\%  & 15.19\% & 12.31\% & \textbf{96.97\%} & 635.30 & 121.74 & 121.77 & 201.99 & \textbf{0.65 (187.29$\times$)} \\
        \hline
        Airtel2-1 & 6.88\% & 18.12\% & 18.23\% & 17.46\% & \textbf{82.64\%} & 171.85 & 121.55 & 121.56 & 201.90 & \textbf{0.60 (202.58$\times$)}\\
        \hline
        Airtel1-2 & 4.89\% & 13.20\% & 11.76\% & 10.67\% & \textbf{85.50\%} & 1488.84 & 122.25 & 122.44 & 202.11 & \textbf{4.99 (24.50$\times$)}\\
        \hline
        Airtel2-2 & 1.49\% & 10.73\% & 9.69\% & 6.93\% & \textbf{73.38\%} & 924.10 & 127.78 & 129.81 & 215.54 & \textbf{73.64 (1.74$\times$)}\\
        \hline
        B4-2013 & 0.04\% & 7.96\% & 7.96\% & 7.70\% & \textbf{79.80\%} & 831.54 & 63.65 & 63.23 & 111.79 & \textbf{22.17 (2.85$\times$)} \\
        \hline
        B4-2018 & 0\% & 5.74\% & 5.74\%  & 3.41\% & \textbf{72.72\%} & 1129.54 & 83.37 & 82.72 & 147.73 & \textbf{89.69 (0.92$\times$)}\\
        \hline
        BT North America & 0\% & 16.98\% & 15.87\% & 7.99\% & \textbf{83.38\%} & 1000.06 & 39.17 & 39.28 & 86.38 & \textbf{7.78 (5.03$\times$)}\\
        \hline
        NTT & 0\% & 6.73\% & 6.49\% & 3.5\% & \textbf{75.94\%} & 911.03 & 120.79 & 118.67 & 196.74 & \textbf{26.88 (4.41$\times$)}\\
        \hline
        OTEGlobe & 0.39\% & 0.38\% & 0.39\% & 0.20\% & \textbf{80.16\%} & 645.92 & 120.92 & 116.18 & 248.62 & \textbf{9.48 (12.26$\times$)}\\
        \hline
	    Fattree ($k=48$) & 31.16\% & 100\% & Memory Out & Time Out & \textbf{96.81\%} & 25.42 & 0.71 & Memory Out & Time Out & \textbf{0.12 (5.92$\times$)}\\
        \hline
	    LONet & 0.01\% & 100\% & Memory Out & Time Out & \textbf{96.81\%} & 228.61 & 1.97 & Memory Out & Time Out & \textbf{0.12 (16.42$\times$)}\\
	   \hline
    \end{tabular}
    }
    \caption{The verification time of incremental update.}
    \label{fig:incremental}
% \vspace{-2em}
% \end{table*}






==> incremental-evalution2.tex <==
%\section{The verification time of incremental update}

\begin{table*}[]
    \centering
\footnotesize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
	    \hline
	    \multirow{2}{*}{\textbf{Network}} & 
	    \multicolumn{5}{c|}{85\% quantile} &
	    \multicolumn{5}{c|}{90\% quantile}  \\
	    \cline{2-11}
         &  \textbf{AP} & \textbf{APKeep} & \textbf{Delta-Net} & \textbf{VeriFlow} & \textbf{DDPV}
         &  \textbf{AP} & \textbf{APKeep} & \textbf{Delta-Net} & \textbf{VeriFlow} & \textbf{DDPV} \\
        \hline
         \multirow{2}{*}{Internet2} & \multirow{2}{*}{3063.64} & \multirow{2}{*}{36.66} & \multirow{2}{*}{36.67} & \multirow{2}{*}{61.09} & \textbf{testbed: 34.81(1.05$\times$)} & \multirow{2}{*}{3716.39} & \multirow{2}{*}{38.13} & \multirow{2}{*}{38.17}  & \multirow{2}{*}{61.26} &  \textbf{ 68.61 (0.56$\times$)} \\
        & & & & & \textbf{simulation: 53.65(0.68$\times$)} & & & & &  \textbf{141.02 (0.27$\times$)}\\
        \hline
        Stanford & 13683.64 & 0.29 & 1.73 & 0.52 & \textbf{0.22(1.32$\times$)} & 19030.97 & 0.33 & 2.08 & 0.69 & \textbf{1.12(0.29$\times$)} \\
        \hline
        Airtel1-1 & 726.56 & 122.08 & 122.17 & 202.01 & \textbf{0.74(164.97$\times$)} & 822.71 & 125.38 & 125.56 & 208.68 & \textbf{0.98(127.94$\times$)} \\
        \hline
        Airtel2-1 & 189.14 & 121.74 & 121.80 & 201.91 & \textbf{154.15(0.79$\times$)} & 207.13 & 122.17 & 122.09 & 205.66 & \textbf{269.71(0.45$\times$)} \\
        \hline
        Airtel1-2 & 1635.36 & 123.07 & 123.10 & 208.58 & \textbf{5.29(23.26$\times$)} & 1833.77 & 127.07 & 128.72 & 208.89 & \textbf{199.12(0.64$\times$)} \\
        \hline
        Airtel2-2 & 983.32 & 130.59 & 131.18 & 224.92 & \textbf{131.98(0.99$\times$)} & 1065.13 & 132.05 & 135.14 & 233.70 & \textbf{207.55(0.64$\times$)} \\
        \hline
        B4-2013 & 888.23 & 110.49 & 110.49 & 184.15 & \textbf{47.72(2.32$\times$)} & 953.20 & 111.85 & 111.86 & 192.72 & \textbf{63.10(1.77$\times$)} \\
        \hline
        B4-2018 & 1219.61 & 83.60 & 83.33 & 153.32 & \textbf{124.65(0.67$\times$)} & 1318.77 & 83.84 & 84.68 & 164.73 & \textbf{141.92(0.59$\times$)} \\
        \hline
        Bt North America & 1119.40 & 39.91 & 40.90 & 97.37 & \textbf{16.14(2.47$\times$)} & 1261.01 & 41.66 & 41.00 & 107.11 & \textbf{35.47(1.16$\times$)} \\
        \hline
        Ntt & 1025.13 & 123.35 & 121.66 & 211.71 & \textbf{39.10(3.11$\times$)} & 1150.51 & 131.14 & 129.40 & 220.83 & \textbf{99.75(1.30$\times$)} \\
        \hline
        OTEGlobe & 698.13 & 124.17 & 118.80 & 259.73 & \textbf{24.18(4.91$\times$)} & 773.15 & 126.25 & 122.65 & 272.82 & \textbf{40.26(3.05$\times$)} \\
        \hline
        Fattree ($k=48$) & 27.66 & 0.72 & Memory out & Time out & \textbf{0.14(5.14$\times$)} & 32.86 & 0.75 & Memory out & Time out & \textbf{0.15(5.00$\times$)} \\
        \hline
        LONet & 314.33 & 1.99 & Memory out & Time out & \textbf{0.14(14.21$\times$)} & 394.74 & 2.02 & Memory out & Time out & \textbf{0.15(13.47$\times$)}\\
        \hline
    \end{tabular}
    \caption{The verification time of incremental update (milliseconds).}
    \label{tab:incremental2}
% \vspace{-3em}
\end{table*}


==> lang-new.tex <==
\section{New Specification Language}
\begin{figure}[t]
\centering
%\footnotesize
\begin{tabular}{rcll}
%	$prog$ & $::=$ & $[s_1; \ldots; s_n]~[req_1; \ldots;
%	req_n]~\mathbf{verify}~req;$  \\
%	$s$ & $::=$ & $sid: s\_pred |~\{sid\}^+$ \\
%	$s\_pred$ & $::=$ & $packet\_space~|~(packet\_space, ingress\_points)$ \\
%              & $|$ & $(packet\_space, egress\_points)$ \\
%	      & $|$ & $(packet\_space, ingress\_points, egress\_points)$ \\
%	$packet\_space$ & $::=$ &\\
%	$ingress\_location$ & $::=$ &\\
%	$egress\_location$ & $::=$ &\\

  \emph{reqs} & $::=$ & $\var{req}^*$ \\
  $\var{req}$ & $::=$ & $(ps, req\_pred)$ & \\
	 $ps$	      & $::=$ & $id$: $packet\_space, ingress\_set$ & \\
	 $req\_pred$  & $::=$ & $[path, req\_context]$ & \\
		      & $|$ & $[id1, id2, comp\_context]$ &\\
	              & $|$ & $req\_pred$ \textbf{or} $req\_pred$ & \\
		      & $|$ & $req\_pred$ \textbf{and} $req\_pred$ & \\
	$path$ & $::=$ & $path$ $path$ & \\
	              & $|$ & $path$ $\shortmid$ $path$ & \\
		      & $|$ & \textbf{not} $path$ &  \\
		      & $|$ & $path^*$ &\\
			& $|$ & $dev$ \\
			& $|$ & $.$ \\
	$req\_context$ & $::=$ & $\mathbf{exist}~count\_exp $ | $\mathbf{equal}$ &\\    
%	$\var{hop}$ & $::=$ & $.$ | $dev$ | $!$ | $dev \shortmid dev$  & \\
%      & $|$ & . &  \\
%    	& $|$ & * & \\
$count\_exp$ & $::=$ & $== N$ | $>= N$ | $> N$ | $<= N $ | $< N $ &   \\
	$comp\_context$ & $::=$ & $\mathbf{ndisjnt}$ | $\mathbf{edisjnt}$ 
  |  $\mathbf{sym}(path \shortmid *)$ &  
%	& $|$ & $\hat{ }$ & (\textsc{Start of Path}) \\
%    	& $|$ & \$ & (\textsc{End of Path}) \\
%         & $|$ & > & (\textsc{Packet Destination}) \\
\end{tabular}
	\caption{The abstract syntax of the \system{} requirement specification
	language.}
\label{fig:grammar-new}
\end{figure}











==> property.tex <==
\section{Verification property comparison}

\begin{table}[!htbp]
    \centering
\footnotesize
    \begin{tabular}{|c|c|}
	        \hline
        \textbf{Reachability} & \\
               \hline
	    \textbf{Loop-freeness} & \\
\hline
        \textbf{Black hole freness} & \\
	\hline
        \textbf{Waypoint} & \\
	   \hline
	\textbf{Mulicast reachability} & \\
	    \hline
	\textbf{Anycast reachability} & \\
	    \hline
	\textbf{1+1 routing} & \\
	   \hline
	\textbf{Full reachability} & \\
	   \hline
	\textbf{Full, shortest-path reachability} & \\
	   \hline
	Route symmetry & \\
	   \hline
	Route disjointness & \\
	
        \hline

    \end{tabular}
    \caption{Verification capability}
    \label{tab:property}
\end{table}













==> related-work.tex <==
\section{Related Work}\label{sec:related-work}
Network verification is usually categorized into (1) control plane
verification (CPV) that finds errors in configuration files~\cite{bagpipe, batfish, minesweeper,
ali-sigcomm20, era-osdi16, bonsai, shapeshifter, gember2016fast, arc-sosp17,
tiramisu, plankton-nsdi20, netdice-sigcomm20, nv-pldi20}; and (2) DPV that checks the
correctness of the data plane, which is the focus of \system{}. 
Simulation based CPV tools~(\eg, \cite{batfish,
liu2017crystalnet, lopes2019fast}) can also benefit from \system{} to verify the simulated data planes.


\para{Centralized DPV.}
Many DPV tools are designed~ \cite{xie2005static, flowchecker,
anteater, hsa, nod, netplumber, veriflow, deltanet-nsdi17, ap-icnp13, ap-ton16,
practical-ap-conext15, practical-ap-ton17, scalable-ap-ton17, apkeep-nsdi20}.
They all use a centralized server to collect the
data planes from all network devices and analyze them. Despite substantial
efforts on performance optimization, the centralized design makes them
unscalable in nature, in that (1) it requires reliable connections between the
server and network devices, and (2) the server becomes both a performance
bottleneck and a single point of failure. In contrast, \system{} adopts a
distributed design, which systematically decomposes the job of DPV into smaller
tasks executed at devices, achieving scalable data plane correctness checkups. 

\para{Scaling up DPV.}
Several designs explore how to scale DPV~\cite{symmetry, libra, azure}. Plotkin \textit{et al.}~\cite{symmetry} exploits the symmetry and
surgery in topology to aggregate  network to a smaller one, but requires data
planes at devices to be isomorphic.  Libra~\cite{libra}
parallels the verification by partitioning headers into subspaces.  Its packet
space decomposition is orthogonal to the topology decomposition of
\system{}. Two can be integrated to further scale up DPV. The only known DPV tool
decomposing verification to local tasks is RCDC in  
Azure~\cite{azure}. It lets devices to locally verify its
data plane, but only for the availability
and fault-tolerance of shortest paths. \system{} is a more  generic
framework that can verify a wide range of 
requirements distributively,
including RCDC as a special case.

\para{Verification of stateful / programmable DP.} 
Other than verifying the data plane generated by routing protocols, some studies
also investigate the verification of stateful data planes (\eg, middleboxes) 
~\cite{panda2017verifying, zhang2020automated, zaostrovnykh2017formally} and
programmable data planes (\eg, P4~\cite{bosshart2014p4})~\cite{liu2018p4v,
dumitrescu2020bf4}. Investigating how \system{} can be extended to support
verifying stateful and programmable data planes would be an interesting future
work.

\para{Data plane synthesis.}
DP synthesis tools~\cite{merlin, contra, propane, el2017network,
el2018netcomplete}  compute  device configurations (\eg, routing protocol
configurations and programmable data plane) that will generate data planes
satisfying the specified intents. \system{} is inspired by several such
tools~\cite{merlin, propane, contra} to use the automata theory to
generate \dvnet{}, a compact representation of all valid paths
%in the network allowed by requirement.

\para{Predicate representation.}
\system{} chooses BDD~\cite{bryant1986graph} as the predicate representation
because state-of-the-art DPV tools show that it is  efficient predicates. Compared with BDD, recent data structures such as
ddNF~\cite{bjorner2016ddnf} and \#PEC~\cite{horn2019precise}) may potentially
improve the performance of predicate operations, hence can benefit \system{}. We
leave this as future work.





























==> subset-proof.tex <==
\subsection{Decomposition and Minimal Counting Information of $\mathbf{subset}$ Operator}
As noted in \S\ref{sec:lang}, the \system{} specification language provides a
third $match\_op$ called $\mathbf{subset}$ as a convenience feature. A behavior
$\mathbf{subset}\hspace{0.5em}path\_exp$ is a shortcut of $(\mathbf{match}$
$>=1\hspace{0.5em}path\_exp)$ $\mathbf{and~(match}$ $==0$ $.^*$ $\mathbf{and}$
$(\mathbf{not}$ $path\_exp))$. One way to decompose such a behavior is to
construct separate \dvnet{}s and let devices count them separately. However, 
this behavior allows a more efficient decomposition. Specifically, we construct
one single \dvnet{} representing all valid paths in the network that match
$path\_exp$. After that, each node $u$ in this \dvnet{} computes $\mathbf{c}_u$
using Equations~(\ref{eqn:count-all})(\ref{eqn:count-any}), and also checks 
\qiao{this is incorrect, because a node forwarding outside \dvnet{} doesn't
mean it will reach the destination. It could stop somewhere.}













==> theory.tex <==
\section{Theoretical analysis}

Proof roadmap:

\begin{itemize}
	\item Centralized, backward  counting along \dvnet{} is correct;
\item Single event, sync, DV protocol is correct;
\item Single event, async, DV protocol is correct;
\item Multi-event, async, DV protocol is correct (eventual consistency).
\end{itemize}













==> time-series.tex <==
\section{Time series diagram of CPU load}

\begin{figure*}[t]
    \centering
	\begin{subfigure}[t]{0.32\linewidth}
	    \centering\includegraphics[width=1\linewidth, height=3cm]{figures/eval/mellanox-time-series.png}
		\caption{\label{fig:time-cpu-mellanox} Mellanox.}
	\end{subfigure}
\hfill
	\begin{subfigure}[t]{0.32\linewidth}
	    \centering\includegraphics[width=1\linewidth, height=3cm]{figures/eval/p4-time-series.png}
		\caption{\label{fig:time-cpu-p4} Barefoot.}
	\end{subfigure}
\hfill
	\begin{subfigure}[t]{0.32\linewidth}
	    \centering\includegraphics[width=1\linewidth, height=3cm]{figures/eval/polaris-time-series.png}
		\caption{\label{fig:time-cpu-polaris} Polaris.}
	\end{subfigure}
	\caption{Time series diagrams of CPU load on three switches as router yoza\_rtr from Stanford network.}
	\label{fig:time-series}
\end{figure*}

\begin{figure*}[t]
    \centering
	\begin{subfigure}[t]{0.32\linewidth}
	    \centering\includegraphics[width=1\linewidth, height=3cm]{figures/eval/ft_core.png}
		\caption{\label{fig:time-cpu-core} Core switch.}
	\end{subfigure}
\hfill
	\begin{subfigure}[t]{0.32\linewidth}
	    \centering\includegraphics[width=1\linewidth, height=3cm]{figures/eval/ft_aggregation.png}
		\caption{\label{fig:time-cpu-aggregation} Aggregation switch.}
	\end{subfigure}
\hfill
	\begin{subfigure}[t]{0.32\linewidth}
	    \centering\includegraphics[width=1\linewidth, height=3cm]{figures/eval/ft_edge.png}
		\caption{\label{fig:time-cpu-dege} Edge switch.}
	\end{subfigure}
	\caption{Time series diagrams of CPU load on Mellanox switch as three kinds of routers from FatTree network.}
	\label{fig:time-series-ft}
\end{figure*}

We run initialization experiment on three switches respectively, and time series diagrams of CPU loads measured by top are presented in Figure \ref{fig:time-series}.

We choose one router from each of the three types in FatTree network, and test the CPU load on the Mellanox switch during initialization, as shown in Figure \ref{fig:time-series-ft}.





==> veri-and-req.tex <==
\para{Verification, requirements, and behaviors.} 
%\dduan{This section is a bit more rigorous now. Do you think it needs one more step for clarification to make it easier to understand?}
We now use the framework of packet traces and universes to reason about data
plane verification. Specifically, the problem of data plane verification 
checks whether certain
\textit{requirements} are met, where each requirement specifies that the set of
all universes of a packet $p$ from ingress $S$ satisfy a set of desired
\textit{behaviors}.
Here, behaviors can be modeled as predicates over the sets of universes (\ie, a
behavior assigns truth values to sets of universes). For the sake of this
paper, given the set of all universes of $p$ entering the network from ingress $S$, 
we consider two forms of behaviors:
\begin{itemize}[leftmargin=*]
\setlength\itemsep{0em}
\item (Existence): Does each universe of $p$ contain 
a certain number of packet traces that match a desired pattern?

%	at
%	least $n$ (or at most $n$, or exactly $n$) traces that match a desired
%		pattern?
%\qiao{we need to discuss a bit about this, the grammar
%we had is more generic, and I'm considering adding another
%syntax sugar on top of it.} 
\item (Equivalence): Does the union of all universes of $p$ equal to the set of
	all paths in the network that satisfy a desired pattern?
\end{itemize}
% \begin{itemize}[leftmargin=*]
% 		\setlength\itemsep{0em}
% \item (Existence requirement): In each universe of $p$ (entering the network at $S$), are there at least $n$ traces that satisfy a desired behavior $B$?
% \item (Equivalence requirement): Does the union of all universes of $p$ (entering the network at $S$) consist of all traces that satisfy a desired behavior $B$?
% \end{itemize}

These behaviors can be used to form a wide range of requirements in data plane
verification. For example, the existence behavior can be used to express
simpler requirements such as reachability, waypoint
reachability, and loop-freeness, which are supported by existing DPV tools~\cite{hsa,
netplumber, veriflow, ap-icnp13, apkeep-nsdi20}, as well as more advanced
requirements, such as multicast, anycast and "no-redundant-delivery" routing.
Another example 
is a requirement given in Azure RCDC~\cite{azure},
which requires that all pairs of ToR devices should reach each other along a shortest
path, and all ToR-to-ToR shortest paths should be available in the data plane.
This can be formulated as a conjunction of an equivalence behavior satisfying
all shortest paths across all universes and an existence behavior satisfying
that at least one shortest path is available in each universe. 
Next, we will explore how \system{} expresses requirements and behaviors in greater detail.


\iffalse{
existence requirements and equivalence requirements, respectively. Existence
requirements include simpler requirements such as reachability, waypoint
reachability,
and loop-freeness, which are supported by existing DPV tools~\cite{hsa,
netplumber, veriflow, ap-icnp13, apkeep-nsdi20}, as well as more advanced
requirements, such as multicast, anycast and "no-redundant-delivery" routing.
Another example 
is a requirement given in Azure RCDC~\cite{azure},
which requires that all pairs of ToR devices should reach each other along a shortest
path, and all ToR-to-ToR shortest paths should be available in the data plane. This can be formulated as an equivalence requirement where each path expression matches the corresponding shortest ToR-ToR paths for the given packet/ingress.
In Section~\ref{sec:lang}, we will explore how \system{} expresses requirements and behaviors in greater detail. 
}\fi

%the shortest path reachability and fault-tolerance requirement



%(1) $p$ can all traces in the same universe can simultaneously happen; 
%(2) $p$ cannot simultaneously have two different traces from different
%universes;

%cannot happen simultaneously
%traces} is defined as a set of traces




==> workflow.tex <==

\subsection{Workflow}\label{sec:workflow}
We demonstrate the workflow of \system{} with an example in
Figure~\ref{fig:workflow-example}. Specifically, we consider a network topology
in Figure~\ref{fig:workflow-topo} and the following requirement: for all
packets destined to 10.0.0.0/23, when they enter the network from $S$, they
must be able to reach $D$ (\ie, reachability), which is the device with an external port
reachable to 10.0.0.0/23, via a simple (\ie, loop-free) path bypassing device
$W$ (\ie, waypointing).

\para{From requirement to \dvnet{}.} 
After this requirement is sent to the verification planner, the planner
multiplies the regular expression in $path\_set$ and the network topology to
generate the \dvnet{}, which compactly represents all paths in the network that
satisfy this regular expression (Figure~\ref{fig:workflow-dvnet}). 
Notice that 
nodes in \dvnet{} do not necessarily map 1-to-1 to devices in the network.
For example, device $C$ is split into nodes $C1$ and $C2$, because the regular
expression allows packets to reach $D$ via $[C, W, D]$ or $[W, C, D]$. \dduan{In general, will this always be many-1, or might it sometimes be many-many?}

With the computed \dvnet{}, the problem of verifying whether the data plane of
the network (Figure~\ref{fig:workflow-fib}) satisfies the given requirement is
transformed to the problem of counting whether at least 1 copy of $p$
destined to 10.0.0.0/23 is delivered to $D1$ in all of $p$'s universes. The planner
then decomposes this job into a series of counting tasks, which are
executed on corresponding devices. 
%\qiao{whether or not emphasize bakcwards?}

\para{Backward, distributed counting along \dvnet{}.} 
Figure~\ref{fig:workflow-dvnet} illustrates the distributed counting process.
For simplicity, we use $P_1, P_2, P_3$ to represent the packet spaces with
destination IP prefixes of $10.0.0.0/23$, $10.0.0.0/24$, and $10.0.1.0/24$,
respectively. Notice that $P_2 \cap P_3 = \emptyset$  and $P_1 = P_2 \cup P_3$.
Given a node in \dvnet{}, the algorithm uses the data plane of its corresponding device in
the network and the results of the counting tasks from all its downstream
neighbor nodes as input, and computes a $packet~space \mapsto count$ mapping. \dduan{Does it use the data plane here or the LEC table as input?} \qiao{LEC, I realized that I only mentioned LEC in 2.3, but not here...} For a given packet space, this
mapping records the number of packet copies in all
universes that can reach from the current node to the destination node in
\dvnet{}. \dduan{The packet spaces here really form a partition of the entire packet space, right? And the packet spaces are determined by a device's LECs (and potentially are further divided by downstream LECs)?} \qiao{Yes.} 

Each node stores its computed  mapping in the CIB of its corresponding device,
and sends it to the devices of upstream neighbors of the current node. For
example, after node $D1$ computes its mapping $[P_1, 1]$ (\ie, one copy of any
packet in $P_1$ will be sent to the correct external ports), it sends this
result to $W$ and $C$, the devices of its upstream neighbors $W1$, $W2$, $W3$
and $C1$. \dduan{This language makes it sound like the nodes in dvnet are physical things communicating with each other, but it's really still the local verifiers communicating, right?} \qiao{yes, we need to clarify the connection in DVNet is logical connection.} Because $C1$ only has one downstream neighbor $D1$, $C1$ checks the
data plane of $C$, computes its mapping also as $[P_1, 1]$, and sends to $W$,
the device of its upstream neighbors $W1$ and $W3$. As a result of this
backward counting process, the ingress device $S$ will eventually receive the
complete counting result as the final verification result. 

In this example, the verification requirement is not satisfied by the data plane
in Figure~\ref{fig:workflow-fib}. We provide details on the mapping computation
at node $A1$ to illustrate how the counting process in \system{} captures this
error. When $A1$ receives the mapping $[(P_1, 0)]$ from $B1$ and $[(P_1, 1)]$
from $W3$, it examines the data plane at device $A$. It finds that for predicate
$P_3$, because $A$ forwards all packets in $P_3$ to $W$, the count of copies of
every packet in $P_3$ can be delivered from $A$ to $D$ is 1. However, for
packets in predicate $P_2$, $A$'s action is to forward them to either $B$ or
$W$, but not both. As such, in one universe where $A$ forwards packets in $P_2$
to $B$, the count of copies delivered to $D$ is 0. In the other universe where
$A$ forwards packets in $P_2$ to $W$, the count is 1.  Therefore, the mapping
$A1$ records for $P_2$ is $(P_2, [0, 1])$, indicating that in one universe,
there will be zero packets in $P_2$ delivered to $D$ by $A$. Once such information is
received by $S1$, because $S$ forwards $P_1$ to $A$, $S$ can capture this error
and alert the operators.

\para{Handling incremental data plane updates.}  
\dduan{Does this step involve the centralized planner (no, right?). If not, then I think that's an important thing to note (when the planner is involved) and is only involved when the requirements or topology change (not when forwarding rules are changed?). Maybe this will address some of the review comments point out that ddpv still uses a centralized component} \qiao{yes, a sentence here should help, and I think we should add another paragraph in Sec. 3 related to this point.}
We complete the workflow demonstration of \system{} by considering a scenario
where $B$ updates its data plane to forward $P_1$ to $W$, instead of to $C$.
The changed mappings of different nodes are circled with boxes in
Figure~\ref{fig:workflow-dvnet}.  In this case, $B1$ and $B2$ will each update
their mappings to $[(P_1, 1)]$ and $[(P_1, 0)]$, respectively, and send the update
to the devices of their upstream neighbors.  However, $B2$'s upstream neighbor
$W3$ does not need to update its mapping because $W$ does not forward any packets
to $B$. In contrast, $B1$'s upstream neighbor $A1$ will update its mapping to
$[(P_1, 1)]$ because (1) no matter whether $A$ forwards packets in $P_2$ to $B$ or $W$,
1 copy of each packet will be sent to $D$, and (2) $P_2 \cup P_3 = P_1$.
Similarly, $S1$ will update its mapping to $[(P_1, 1)]$ as well, \ie, the
requirement is satisfied after the update.% data plane. 

\para{Why backward counting instead of forward counting?}
Readers may think of using distributed forward counting along \dvnet{} to perform verification. Intuitively, compared with backward counting in \system{}, this appears to be more natural. However, in order to verify a requirement with more than one $path\_exp$ with a consistent result, such as multicast and anycast, the system needs an "aggregation" point to collect the counting result of multiple $path\_exp$s. Because using backward counting, 
\qiao{unfinished, needs to think more}
Second reason, incremental update? Third, support fast reroute??



\iffalse{
\qiao{where do we put this paragraph? Maybe in introduction?}
\system{} achieves fast, scalable data plane verification for two reasons.
First, by decomposing a centralized verification task into smaller counting
tasks executed on devices, the verification latency of \system{} achieves a
scalability approximately linear to the diameter of the network. 
Second, when a data plane update happens, only devices whose counting results
may change need to incrementally update their results. In our experiments, the
number of such devices is far smaller than the total number of devices in the
whole network.
}\fi




%Different from centralized EC-based DPV tools, \system{} handles




%\para{Summary.}
















